Retrospective Loss: Looking Back to Improve Training of Deep Neural Networks

Deep neural networks (DNNs) are powerful learning machines that have enabled breakthroughs in several domains. In this work, we introduce a new retrospective loss to improve the training of deep neural network models by utilizing the prior experience available in past model states during training. Minimizing the retrospective loss, along with the task-specific loss, pushes the parameter state at the current training step towards the optimal parameter state while pulling it away from the parameter state at a previous training step. Although a simple idea, we analyze the method as well as to conduct comprehensive sets of experiments across domains - images, speech, text, and graphs - to show that the proposed loss results in improved performance across input domains, tasks, and architectures.

==> related_work.tex <==
\section{Related Work}
\label{sec_related_work}
% \vspace{-8pt}

The proposed loss leverages parameter states from previous training steps as guidance to compute the current weight update. While there is no explicit effort that implements this idea when training DNN models, one could find similarities with efforts in optimization that utilize information from past training steps for current weight updates. Techniques such as SVRG \citep{svrg}, SARAH\citep{sarah}, and ProxSARAH \citep{ProxSARAH} use gradients from earlier training steps to predict better weight updates. These methods are very different in their objectives, and most often seek to reduce variance in the stochastic gradient descent update. Other optimization methods like Momentum \citep{momentum}, Adam \citep{adam},  Nesterov Momentum \citep{nag} accumulate past gradients to accelerate weight updates in the right direction in order to achieve faster convergence. While these methods leverage the most recent updates to provider a stronger gradient direction, in contrast, our work seeks to leverage the relatively poorer performance of past models states during training. The proposed method can be used to improve performance when used with different optimizer configurations (including Adam or momentum), as shown in our results.

Another genre of efforts could be traced to reinforcement learning (RL), where techniques involve optimizing using moving targets. In such settings, methods for Q-learning and policy gradients benefit from using a guidance network during training. The DQN algorithm proposed by \citep{mnih-nature} uses an additional target network for Q-value updates, where parameters are updated by copying from the additional network at discrete steps. Double Q-learning \citep{double-qn} learns two Q functions, where each Q-function is updated with a value for the next state from the other Q-function. Policy gradient methods such as TRPO \citep{TRPO}, PPO \citep{PPO} use a KL-divergence objective during training that constrains the loss to ensure deviation from a previously learned policy is small. In these techniques, leveraging a guidance during training results in improved convergence and sample efficiency. We note that these efforts, while similar in a sense, are constrained to the RL setting, and the proposed work is the first such effort in supervised learning to the best of our knowledge. Further, the objective in the RL setting is to control divergence from a guidance step to better handle moving targets, which is fundamentally different from the objectives in supervised learning. We note additionally that while the proposed retrospective loss is intended to be added to any task-specific loss, it is not a regularizer (not intended to overcome overfitting), but to improve efficiency and efficacy of DNN model training.


